Patching Weak Convolutional Neural Network Models through Modularization and Composition

Despite great success in many applications, deep neural networks are not always robust in practice. For instance, a convolutional neuron network (CNN) model for classification tasks often performs unsatisfactorily in classifying some particular classes of objects. In this work, we are concerned with patching the weak part of a CNN model instead of improving it through the costly retraining of the entire model. Inspired by the fundamental concepts of modularization and composition in software engineering, we propose a compressed modularization approach, CNNSplitter, which decomposes a strong CNN model for $N$-class classification into $N$ smaller CNN modules. Each module is a sub-model containing a part of the convolution kernels of the strong model. To patch a weak CNN model that performs unsatisfactorily on a target class (TC), we compose the weak CNN model with the corresponding module obtained from a strong CNN model. The ability of the weak CNN model to recognize the TC can thus be improved through patching. Moreover, the ability to recognize non-TCs is also improved, as the samples misclassified as TC could be classified as non-TCs correctly. Experimental results with two representative CNNs on three widely-used datasets show that the averaged improvement on the TC in terms of precision and recall are 12.54% and 2.14%, respectively. Moreover, patching improves the accuracy of non-TCs by 1.18%. The results demonstrate that CNNSplitter can patch a weak CNN model through modularization and composition, thus providing a new solution for developing robust CNN models.

==> variant.tex <==
\input{variant_algo}
\hy{is it used?} \qi{Previously, ICSE papers had not been published, so I designed a variant of FSE for comparison. Maybe this variant is no longer needed?}
As mentioned in Section \ref{sec:related_work}, since the neurons associated with a feature map share the same set of weights determined by the convolution kernel, the neuron activation-based method proposed in \cite{fse2020modularity} cannot be directly applied to CNNs. 
We propose a variant of the method to verify whether the neuron activation can be applied to decompose a CNN model. Same to \cite{fse2020modularity}, the variant decomposes a CNN model by identifying the weights (i.e., convolution kernels) responsible for a concern. 
Since the weights corresponding to an activated neuron are responsible for a concern \cite{fse2020modularity}, a convolution kernel is responsible for a concern if there is a positive value in the feature map produced by the kernel. 
The variant calculates the average of all values in a feature map processed by ReLU to determine whether the kernel is responsible for a concern. 
The variant has two steps including concern identification ($CI$) and tangling identification ($TI$).  Since modularity does not change the output layer (i.e., FC layer) of the CNN model, the variant does not include the third step in \cite{fse2020modularity}, concern modularization, which is used to modify the weights of the output layer. The results of \cite{fse2020modularity} demonstrate that using $CI$ and $TI$ can achieve acceptable results; thus we believe that the variant is sufficient to verify whether the neuron activation can be used to decompose a CNN model. 

The algorithm of the variant is shown in Algorithm \ref{algo:variant}. The inputs of the variant are the pre-trained CNN model ($model$) with $L$ convolutional layers, the data ($X$) and labels ($Y$) of the training set, and the concern ($class$), respectively. 
The output is a two-dimensional array, $idx_k$, that gives which kernels are retained in each convolutional layer. 
Specifically, the kernels are extracted from $model$ (line \ref{algo:variant:extract}) and then indexed using a two-dimensional array $idx_K$ (line \ref{algo:variant:index}). The first dimension of $idx_K$ represents the index of the convolutional layer, and the second dimension represents the index of the kernel. If the value of an element in $idx_K$ is 1, the kernel corresponding to the element is retained; otherwise, the kernel is removed. 

The variant uses $CI$ to identify the kernels corresponding to $class$ and retain the common kernels that are used by all examples belonging to $class$ (line \ref{algo:variant:call_CI}). If for some inputs, the common kernels for all the examples that belong to $class$ are very few, then the retained kernels are too few to construct a good module. To avoid such circumstances, $indicator$ is used to stop $CI$ removing kernels once the number of retained kernels reaches a threshold (lines \ref{algo:variant:indicator_start}-\ref{algo:variant:indicator_end}). 
With every sample labeled $class$, $CI$ extracts the feature maps of the kernels and computes the average of values in each feature map (lines \ref{algo:variant:extract_map}-\ref{algo:variant:mean_fm}). 
If the average value is negative, the value in $idx_K$ corresponding to the kernel that produces the feature map is set 0, meaning the kernel is removed (lines \ref{algo:variant:remove_start}-\ref{algo:variant:remove_end}). 
If the average value is positive and $indicator$ is $true$, the value in $idx_K$ corresponding to the kernel is set to 1, meaning the kernel is retained (lines \ref{algo:variant:add_start}-\ref{algo:variant:add_end}). 

If a module is composed of the common kernels corresponding to a concern, it can only classify the single concern since all the kernels corresponding to the other concerns are removed. The module becomes a single-class classifier and predicts the concern irrespective of the input. \cite{fse2020modularity}
To solve this problem, $TI$ is used to identify some kernels back to $idx_K$, which enables the module to identify inputs that do not need classification by the concern.
Specifically, with every sample that is not labeled $class$, $TI$ computes the average of values in each feature map (lines \ref{algo:variant:ti_fm_start}-\ref{algo:variant:ti_fm_end}). 
If the average value is positive, the kernel corresponds to other concerns and is put back to the module. 

==> variant_algo.tex <==
\begin{algorithm}[]
\footnotesize
\caption{A Variant of the neuron activation-based method}
\label{algo:variant}
\begin{algorithmic}[1]
\Procedure{VARIANT}{$model, X, Y, class$}
    \State $K$ = $extract\_kernels(model)$ \label{algo:variant:extract}
    \State $idx_K = K.idx()$ \Comment{A two-dimensional array filled with ones.} \label{algo:variant:index}
    \State $indicator = True$
    \State $X_{class} = X[Y == class]$
    \For{$i$ = 0, 1, ..., $|X_{class}|-1$}
        \State $idx_K$ = $CI(model, X_{class}[i], indicator, idx_K)$ \label{algo:variant:call_CI}
        \If{$count\_ones(idx_K[L]) \leq 0.1 \times |idx_K[L]|$} \label{algo:variant:indicator_start}
            \State $indicator = True$
        \Else
            \State $indicator = False$ \label{algo:variant:indicator_end}
        \EndIf
    \EndFor
    
    \State $other_{class} = set(Y).remove(class)$
    \For{each $n \in other_{class}$}
        \State $X_{other} = X[Y == n]$
        \For{$i=0, 1, ..., |X_{other}|-1$}
            \State $idx_K$ = $TI(model, X_{other}[i], idx_K)$
        \EndFor
    \EndFor
\State \textbf{return} $idx_K$
\EndProcedure

\\

\Procedure{CI}{$model, input, indicator, idx_K$}
    \State $FM = extract\_feature\_maps(model, input)$ \label{algo:variant:extract_map}
    \For{$i = 0, 1, ..., L-1$}
        \For{$j = 0, 1, ..., |FM[i]|-1$}
            \State $v = mean(FM[i,j])$  \label{algo:variant:mean_fm}
            \If{$v \leq 0$} \label{algo:variant:remove_start}
                \State $idx_K[i, j] = 0$ \label{algo:variant:remove_end}
            \Else
                \If{$indicator == True$} \label{algo:variant:add_start}
                    \State $idx_K[i, j] = 1$ \label{algo:variant:add_end}
                \EndIf
            \EndIf
        \EndFor
    \EndFor
    \State \textbf{return} $idx_K$
\EndProcedure

\\

\Procedure{TI}{$model, input, idx_K$}
\State $FM = extract\_feature\_maps(model, input)$ \label{algo:variant:ti_fm_start}
    \For{$i = 0, 1, ..., L-1$}
        \For{$j = 0, 1, ..., |FM[i]|-1$}
            \State $v = mean(FM[i,j])$  \label{algo:variant:ti_fm_end}
            \If{$v > 0$}
                \State $idx_K[i, j] = 1$
            \EndIf
        \EndFor
    \EndFor
    \State \textbf{return} $idx_K$
\EndProcedure
\end{algorithmic}
\end{algorithm}

